Zero-Shot Slot and Intent Detection in Low-Resource Languages

Intent detection and slot filling are critical tasks in spoken and natural language understanding for task-oriented dialog systems. In this work we describe our participation in the slot and intent detection for low-resource language varieties (SID4LR; Aepli et al. (2023)). We investigate the slot and intent detection (SID) tasks using a wide range of models and settings. Given the recent success of multitask-prompted finetuning of large language models, we also test the generalization capability of the recent encoder-decoder model mT0 (Muennighoff et al., 2022) on new tasks (i.e., SID) in languages they have never intentionally seen. We show that our best model outperforms the baseline by a large margin (up to +30 F1 points) in both SID tasks

==> Tables/table_arocr.tex <==
%Please add the following packages if necessary:
%\usepackage{booktabs, multirow} % for borders and merged ranges
%\usepackage{soul}% for underlines
%\usepackage[table]{xcolor} % for cell colors
%\usepackage{changepage,threeparttable} % for wide tables
%If the table is too wide, replace \begin{table}[!htp]...\end{table} with
%\begin{adjustwidth}{-2.5 cm}{-2.5 cm}\centering\begin{threeparttable}[!htb]...\end{threeparttable}\end{adjustwidth}
\begin{table*}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\resizebox{\textwidth}{!}{%
\hspace*{-0.9cm}
\begin{tabular}{lrrrr}\toprule
\textbf{Models/Datasets} &\textbf{Line Based} &\textbf{Word Based} &\textbf{Character Based} \\\midrule
Tesseract \downarrow &53.67 &97.27 &116.53 \\[0.1cm] \hline \\
TrOCR \downarrow  &45.85 &4.33 &12.80 \\[0.1cm] \hline \\
SOTA \downarrow  &12.24 &4.42 &1.08 \\[0.1cm] \hline \\
ArOCR \downarrow  &\textbf{4.12} &\textbf{0.15} &\textbf{0.03} \\
\bottomrule
\end{tabular}
\hspace*{-0.9cm}
}
\end{table*}
